Drone-based AI and 3D Reconstruction for Digital Twin Augmentation

Digital Twin is an emerging technology at the forefront of Industry 4.0, with the ultimate goal of combining the physical space and the virtual space. To date, the Digital Twin concept has been applied in many engineering fields, providing useful insights in the areas of engineering design, manufacturing, automation, and construction industry. While the nexus of various technologies opens up new opportunities with Digital Twin, the technology requires a framework to integrate the different technologies, such as the Building Information Model used in the Building and Construction industry. In this work, an Information Fusion framework is proposed to seamlessly fuse heterogeneous components in a Digital Twin framework from the variety of technologies involved. This study aims to augment Digital Twin in buildings with the use of AI and 3D reconstruction empowered by unmanned aviation vehicles. We proposed a drone-based Digital Twin augmentation framework with reusable and customisable components. A proof of concept is also developed, and extensive evaluation is conducted for 3D reconstruction and applications of AI for defect detection.

==> archived/_abstract.tex <==
\keywords{Digital Twin \and 3D Reconstruction \and Artificial Intelligence (AI) \and Information Augmentation \and Unmanned Aviation Vehicle (UAV)}

\begin{abstract}
Digital Twin is an emerging phenomenon and is at the forefront of Industry 4.0, with the ultimate goal of combining the physical space and the virtual space in either direction. To date, Digital Twin applications have seen success in several fields and domains. While the nexus of various technologies open up new opportunities in Digital Twin, they are limited by the inherent boundary of each, including the Building Information Model used in the Building and Construction industry. An Information Fusion framework, therefore, is much needed to seamlessly fuse information from the variety of technologies involved. This study aims to augment Digital Twin in the Building and Construction industry with the use of AI and 3D reconstruction empowered by unmanned aviation vehicles. We propose a drone-based Digital Twin augmentation framework with reusable and customizable components. A proof of concept is also developed and comprehensive evaluation is conducted for 3D reconstruction and applications of AI for defect detection. 
\end{abstract}

==> archived/_approach.tex <==
\section{Approach}

We introduce our NexBIM with state-of-the-art technologies to provide the next level of experience with BIM. The use of Mixed Reality (MR) enhanced with Artificial Intelligence (AI) creates an impeccable way to interact with BIM for large-scale infrastructure projects. It will ease the learning curve for users with the automation of 3D modeling and defect detection. Furthermore, it will unveil the possibility for precise point-cloud data and high-resolution images for information fusion beyond the geospatial limitations of BIM. The following sections discussed in detail our contributions in 1) Information Fusion (the backbone of NexBIM), 2) 3D reconstruction techniques, and 3) Adaptation of Mixed Reality, 4) Enhancement of Deep Learning and Transfer learning in crack and defect detection.

\subsubsection{Information Fusion}
\subsubsection{3D Reconstruction Techniques}
\subsubsection{Adaptation of Mixed Reality}
\subsubsection{Enhancement of Deep Learning}

==> archived/_background.tex <==
\section{Background}

It is commonly acknowledged that the concept and model of the Digital
Twin were first publicly introduced in 2002 by Grieves in his
presentation as the conceptual model underlying Product Lifecycle
Management \cite{grieves2002conceptual}. Although the term was not
coined at that time, his idea did have all the basic elements of the
Digital Twin: physical space, virtual space, and the information flow
between them. The key enablers of Digital Twin: sensor technologies,
cloud computing, big data, IoT, and artificial intelligence have since
then experienced growth at an unprecedented rate. Recently, the concept
of Digital Twin was formally defined by NASA as a multiphysics,
multiscale, probabilistic, ultra-fidelity simulation that enables
real-time replication of the state of the physical object in cyberspace
based on historical and real-time sensor data.

\subsection{Architecture}\label{architecture}

The basic components of Digital Twin contain at least three dimensions:
physical space, virtual space, and real-time information flow between
the physical space and virtual space
\cite{grieves2002conceptual,tao2018digitald}. Tao et al. extended the
model and proposed that Digital Twin modeling should involve: physical
modeling, virtual modeling, connection modeling, data modeling, and
service modeling \cite{tao2018digital}. From a more structural and
technological viewpoint, Digital Twin consists of sensor and measurement
technologies, Internet of Things, Big Data and Artificial Intelligence
\cite{kaur2020convergence,kusiak2017smart}.

\subsection{Applications}\label{applications}

The applications of DT span various domains from manufacturing,
aerospace to cyber-physical systems, architecture, construction, and
engineering. Examples of Digital Twin applications are given below:

\subsubsection{Digital Twin in
Manufacturing}\label{digital-twin-in-manufacturing}

Perhaps, applications of Digital Twin are most often found in smart
manufacturing. Due to ever-increasing product requirements and rapidly
changing markets, there has been a growing interest in shifting problem
identification and solving to early stages of product development
lifecycle (also known as ``front-loading'') \cite{thomke2000effect}. The
Digital Twin paradigm fits perfectly because virtual replications of
physical products allow early feedback, design changes, quality, and
functional testing without actually entering the production phase.

Tao et al. suggested that a Digital Twin-driven product design process
can be divided into conceptual design, detailed design, and virtual
verification \cite{tao2019digital}. Throughout the process, various
kinds of data such as customer satisfaction, product sales, 3D model,
product functions, and configuration, sensor updates can be integrated
to mirror the life of the physical product to its corresponding digital
twin. With real-time closed-loop feedback between the physical and the
virtual spaces, designers are able to make quick decisions on product
design adjustment, quality control and improve the design efficiency by
avoiding tedious verification and testing.

During production, simulation of production systems, the convergence of
the physical and virtual manufacturing world leads to smart operations
in the manufacturing process including smart interconnection, smart
interaction, smart control, and management. For e.g:
\cite{tao2017digital} proposed a shop-floor paradigm consists of four
components physical shop-floor, virtual shop-floor, shop-floor service
system driven by shop-floor digital twin data, enabled by IoT, big data,
and artificial intelligence. Modeling of machinery, manufacturing steps,
and equipment also help in precise process simulation, control, and
analysis, eventually leading to improvement of the production process
\cite{botkina2018digital}. A similar effort is observed in
\cite{minos2018towards} to evaluate different methods in automated 3D
reconstruction in SME factories. The authors explored the use of
low-cost stereo vision techniques with Simultaneous Localization and
Mapping (SLAM) to generate Digital Twin models of a physical factory
floor and machinery.

The most popular application area in Digital Twin is PHM according to
the number of reports and publications to date \cite{tao2018digital}.
For e.g. \cite{tuegel2011reengineering} reported improvement in the
management of aircraft service life through modeling, uncertainty
quantification, and structural analysis with Digital Twin.
\cite{seshadri2017structural} developed a procedure for structural
health management of damaged aircraft in the Digital Twin context.
Besides aerospace, Digital Twin applications in PHM can also be found in
manufacturing \cite{aivaliotis2019methodology,ghoshal2019integrated}, energy industry \cite{baraldi2015prognostics,marot2020l2rpn} and construction \cite{Baumann2019}.

\subsubsection{Digital Twin in Building and
Construction}\label{digital-twin-in-building-and-construction}

Modeling of physical buildings and landscapes with Digital Twin brought
valuable opportunities to the architecture, construction, and
engineering industry such as improvements in urban planning, city
analytics, environmental analysis, building maintenance, defect
detection, and collaboration between stakeholders. An important concept
in this domain is Building information modeling (BIM) i.e.~a process
involving the generation and management of digital representations of
physical and functional characteristics of places.

Yan et al. proposed a method for the integration of 3D objects and
terrain in BIMs supporting the Digital Twin which takes the accurate
representation of terrain and buildings into consideration
\cite {yan2019integration}. Models developed by such methods are used
for urban planning, city analytics, or environmental analysis.

Nys et al. utilized LiDAR point clouds data and photogrammetric
techniques for automatic reconstruction of 3D city buildings
highlighting closed solids, coherent surface junctions, and perfect
snapping of vertices, etc. The use of CityJSON specifications was also
investigated for better collaboration. Virtual models are then useable
for complex computations such as computational fluid dynamics
\cite{nys2020automatic}

\subsubsection{Digital Twin by Industry
Leaders}\label{digital-twin-by-industry-leaders}

Gartner 2017 predicted that Digital Twin is one of the top ten trending
strategic technologies \cite{Panetta2016}. Digital Twin since 2012 has
entered rapid growth stage considering the current momentum with
applications in several industries and across variety of domains.

NASA and U.S Air Force adopted Digital Twin to improve production of
future generations of vehicles to become lighter while being subjected
to high loads and more extreme service conditions. The paradigm shift
allowed the organisation to incorporate vehicle health management
system, historical data and fleet data to mirror the life of its flying
twin, thus, enabled unprecedented levels of safety and reliability
\cite{glaessgen2012digital}.

The world's 11th busiest airport, the second largest in the Netherlands,
Amsterdam Airport Schiphol built a digital asset twin of the airport
based on building information modeling (BIM). Known as the Common Data
Environment (CDE), Schiphol's Digital Twin solution integrate data from
many sources: building information model (BIM) data; GIS data; and data
collected in real time on project changes and incidents as well as
financial information, documents, and project portfolios. The
information fusion capability of Digital Twin presents opportunities to
run simulations on potential operational failures throughout the entire
complex \cite{Baumann2019}.

Port of Rotterdam built a Digital Twin of the port and used IoT and
artificial intelligence to collect and analyse data to improve
operations. Digital Twin helps to better predict accurately what the
best time is to moor, depart and how much cargo needs to be unloaded.
Further more, real-time access to information enables better predict
visibility and water conditions \cite{Boyles2019}.

\subsubsection{AI in Digital Twin}\label{ai-in-digital-twin}

The rapid adoption of enabling technologies such as IoT, cloud
computing, big data opens up endless opportunities for applications of
AI in Digital Twin. The overall definition of AI dates back to the 50s
and was formally known as intelligent systems. As a multidisciplinary
field, AI encompasses Machine Learning, Data Mining, Computer Vision,
Natural Language Processing, Robotics among many others. AI is promising
as one of the core services in Digital Twin to assist human in decision
making by finding patterns, insights in big data, generation of
realistic virtual models through advanced computer vision, natural
language processing and robotics etc.

Li et al proposed a method that uses a concept of dynamic Bayesian
networks for Digital Twin to build a health monitoring model for the
diagnosis and prognosis of each individual aircraft
\cite{li2017dynamic}. For example, in diagnosis by tracking
time-dependent variables, the method could calibrate the
time-independent variables; in prognosis, the method helps to predict
crack growth in the physical subject by using particle filtering as the
Bayesian inference algorithm.

In production process, \cite{alexopoulos2020digital} introduced a
Digital Twin-driven approach for developing Machine Learning models. The
models are trained for vision-based recognition of parts' orientation
using simulation of Digital Twin models, which then can help to
adaptively control the production process. Additionally, the authors
also proposed a method to synthesize training datasets as well as
automatic labeling via the simulation tools chain and thus reducing
users' involvement during model training.

Chao et al \cite{fan2021disaster} described an insightful vision of
Digital Twin to enable the convergence of AI and Smart City for disaster
response and emergency management. In this vision, the authors listed
four components in Disaster City Digital Twin i.e.~1) multi-data sensing
for data collection, 2) data integration and analytics, 3) multi-actor
game-theoretic decision making, 4) dynamic network analysis, and
elaborated the functions that AI can improve within each component.

Another interesting vision of Digital Twin in Model-Based Systems
Engineering is described in \cite{madni2019leveraging} in which the
realization of Digital Twin is progressively divided into four levels 1)
Pre-Digital Twin, 2) Digital Twin, 3) Adaptive Digital Twin and 4)
Intelligent Digital Twin. In the last two levels: Adaptive Digital Twin
and Intelligent Digital Twin, the authors emphasized the tight
integration of AI in engineering processes for e.g.~in level 3, an
adaptive user interface can be offered by using supervised machine
learning to learn the preferences and priorities of human operators in
different contexts, therefore, support real-time planning and decision
making during operators, maintenance and support; in level 4,
additionally unsupervised machine learning can help discern objects and
patterns in the operational environment and reinforcement learning can
learn from continuous data stream from the environment.

Power networks are the backbone of power distribution, playing a central
economical and societal role by supplying reliable power to industry,
services, and consumers. To improve the efficiency of power networks,
researchers in the Energy industry have also been putting initial effort
into integrating Digital Twin and AI for informed decision-making in
operation, support, and maintenance \cite{marot2020l2rpn}. In
particular, a virtual replication of the power network is developed.
Various time-series measurements from the physical power networks such
as production values, loads, line thermal limits, power flows, etc. are
streamed back to the virtual models. Based on the digital models,
researchers exploit machine learning algorithms such as reinforcement
learning to predict future states of the networks as well as suggest
possible optimal control actions.

==> archived/_conclusion.tex <==
\section{Conclusion}

==> archived/_introduction.tex <==
\section{Introduction}\label{introduction}

The Digital Twin is the virtual replication of a physical object.
Through modelling and real-time data communication, the Digital Twin
simulates the actual properties and behaviours of its physical
counterpart in the physical space, thus, enable learning, reasoning, and
dynamically re-calibrating for improved decision-making
\cite{glaessgen2012digital,grieves2012digital}. The tight and seamless
integration between the physical and virtual space in the Digital Twin
paradigm makes it one of the most promising enabling technologies for
the realization of smart manufacturing and Industry 4.0
\cite{tao2018digital}

To date, Digital Twin applications have seen success in various
industries and domains, including product design, production, prognostic
and health management, building and construction, and many others.
Recent advances in sensor technologies, big data, cloud computing,
social networks, Internet of Things, computer-aided-design, 3D
modelling, and artificial intelligence allow a massive amount of data to
be collected while enabling real-time communication for the realization
of the Digital Twin paradigm throughout the complete product's
life-cycle
\cite{tao2018digital,qi2019enabling,tao2018digitalb, fuller2020digital}.

In the building and construction industry context, physical objects are
buildings and structural components. To generate and capture their
virtual counterparts in the virtual space, Building Information Model
(BIM) is a common standard that encompasses a large amount of detail on
building dimensions and critical components. These components include
façade features, dimensions of staircases, slopes of walls, height of
railings, etc. The use of BIM provides high-quality preconstruction
project visualisation, improved scheduling, and better coordination and
issue management. The Digital Twin paradigm in this industry utilises
BIM as one of the core technologies to facilitate information
management, information sharing, and collaboration among stakeholders in
different domains over the building life cycle
\cite{adamu2015social,das2014bimcloud}.

In many cases, it is often desirable to obtain 3D models of the physical
buildings and landscapes that can be used for enrichment, visualization,
and advanced analytics of Digital Twin models
\cite{minos2018towards,henry2014rgb,spreitzer2020large,dryanovski2017large}.
Additionally, other sources of information can be useful for the Digital
Twin models, such as contextual information and geographical information
systems (GIS). However, there are some limitations with the current BIM
technologies that hinder the capability to integrate multiple sources of
data. For instance, BIM files are restricted in size, making it
difficult to add large artefacts. The BIM format is neither initially
designed for the integration of heterogeneous data sources nor capable
of capturing real-time updates.

The process to obtain 3D models of the physical buildings and landscapes
is also labour-intensive. When 3D reconstruction is done manually using
a hand-held device, the ability to capture an extensive model of the
building is often limited due to physical constraints such as the size
of tunnels or large constructions. These issues call for a new and more
scalable approach in 3D reconstruction using unmanned aerial vehicles
(UAV), optimal scanning methods, and advanced onboard processing
algorithms
\cite{mauriello2014towards,spreitzer2020large,shim2019development}.

On the other hand, real-time applications of AI and image analysis of
BIM is also underdeveloped. One application of imaging in building
maintenance for Digital Twin is defect detection, in which AI algorithms
are employed to recognize defect regions such as cracks automatically.
To develop such AI models, appropriate training data is required which,
however, is often found in 2D format, prompting suitable methods on
real-time transformation for AI applicability.

Motivated by the current limitations of building and construction
technologies, we aim to innovate BIM for Digital Twin in two broad
areas: 1) Develop an Information Fusion framework that extends BIM with
a metadata layer to support heterogeneous data integration; 2) Enhance
real-time synchronization between the physical space and virtual space
in BIM through improved 3D reconstruction methods and real-time
scanning.

To this aim, our approach is four-fold: First, we develop a proof of
concept Information Fusion framework to facilitate the integration of
multiple sources of information to produce useful data representations
for BIM applications. It utilises a distributed and fault-tolerant
database to store geometry objects (e.g., buildings and structural
components) and meta-information (e.g., defects and tagged items) to
provide maximal compatibility and highest/raw details; Second, we build
a drone-based 3D reconstruction solution for scalable data collection
and evaluate major scanning technologies including LiDAR sensor,
stereovision, and single-lens camera; Third, we test our real-time
scanning capabilities by performing real-time 2D to 3D mapping from our
camera feed at five frames per second. The mapping computation is done
on the drone using an onboard miniature computer; Finally, we present a
defect detection use-case as an application of AI in real-time image
scanning.

The contributions of our work are as follows: We provided a
comprehensive review of Digital Twin technologies in conjunction with
AI. We demonstrated an end-to-end proof of concept of the use of BIM for
Digital Twin and information fusion. We conducted extensive experiments
for the evaluation of 3D reconstruction techniques. Finally, we
illustrated the feasibility of AI application in Digital Twin through
defect detection with deep learning use-case. Our work provides valuable
insights and important theoretical and empirical implications for
researchers as well as practitioners in this emerging field.

==> archived/_results.tex <==
\section{Results}
